Weakly-Supervised Visual-Textual Grounding with Semantic Prior Refinement

Using only image-sentence pairs, weakly-supervised visual-textual grounding aims to learn region-phrase correspondences of the respective entity mentions. Compared to the supervised approach, learning is more difficult since bounding boxes and textual phrases correspondences are unavailable. In light of this, we propose the Semantic Prior Refinement Model (SPRM), whose predictions are obtained by combining the output of two main modules. The first untrained module aims to return a rough alignment between textual phrases and bounding boxes. The second trained module is composed of two sub-components that refine the rough alignment to improve the accuracy of the final phrase-bounding box alignments. The model is trained to maximize the multimodal similarity between an image and a sentence, while minimizing the multimodal similarity of the same sentence and a new unrelated image, carefully selected to help the most during training. Our approach shows state-of-the-art results on two popular datasets, Flickr30k Entities and ReferIt, shining especially on ReferIt with a 9.6% absolute improvement. Moreover, thanks to the untrained component, it reaches competitive performances just using a small fraction of training examples.

==> tables/backup_table_fraction_results.tex <==
\begin{table}
  \centering
  \footnotesize
  \begin{tabular}{lcc}
    \toprule
    Training Fraction &\multicolumn{1}{c}{Flickr30k Entities (\%)} & \multicolumn{1}{c}{ReferIt (\%)} \\
    \midrule
    5\%         &$57.20$        &$41.02$ \\
    10\%        &$60.72$        &$42.67$ \\
    50\%        &$61.49$        &$47.68$ \\
    100\%       &$\bm{62.20}$   &$\bm{48.04}$ \\
    \bottomrule
  \end{tabular}
  \caption{\emph{Accuracy} values obtained by our model on Flickr30k Entities and ReferIt test sets. The best values are shown in bold. Our model presents competitive results even when trained with just 5\% of the training set data.}
  \label{tab:table_fraction_results}
\end{table}



% \begin{table*}
%   \centering
%   \small
%   \begin{tabular}{lcccccccc}
%     \toprule
%     &\multicolumn{4}{c}{Flickr30k Entities (\%)} & \multicolumn{4}{c}{ReferIt (\%)} \\
%     \cmidrule{2-5} \cmidrule{6-9}
%     &\multicolumn{2}{c}{Ours} & \multicolumn{2}{c}{MAF} &\multicolumn{2}{c}{Ours} & \multicolumn{2}{c}{MAF} \\
%     \cmidrule(rl{4pt}){2-3} \cmidrule(rl{4pt}){4-5} \cmidrule(rl{4pt}){6-7} \cmidrule(rl{4pt}){8-9}
%     Fraction    & Accuracy & P. Acc. & Accuracy & P. Acc. & Accuracy & P. Acc. & Accuracy & P. Acc. \\
%     \midrule
%     1\%         & & & & & &  & & \\
%     5\%         & & & & & &  & & \\
%     10\%        & $60.72$ & $80.37$ & $60.05$ & $81.94$ & $34.48$ & $58.18$ &$28.05$ &$53.94$ \\
%     50\%        & $61.49$ & $80.15$ &$\bm{61.08}$ &$83.40$ & $\bm{34.63}$ & $\bm{58.26}$ &$\bm{29.09}$ &$\bm{54.75}$ \\
%     100\%       & $\bm{62.20}$ & $\bm{80.68}$ & $60.80$ & $\bm{83.62}$ &$34.61$ &$58.22$ &$28.91$ &$54.61$ \\
%     \bottomrule
%   \end{tabular}
%   \caption[Results on Flickr30k Entities test set]{Results on Flickr30k Entities test set. \textit{Accuracy} is the standard accuracy metric, while \textit{P. Acc.} is the pointing game accuracy metric, both reported in percentage. \todo{Aggiungi i risultati e aggiorna caption. Volendo si possono rimuovere le P.Acc. per guadagnare molto spazio.}}
%   \label{tab:table_fraction_results}
% \end{table*}


==> tables/backup_table_omega.tex <==
\begin{table}
  \centering
  \footnotesize
  \begin{tabular}{lcccc}
    \toprule
    $\omega$ &\multicolumn{1}{c}{Flickr30k Entities (\%)} & \multicolumn{1}{c}{ReferIt (\%)} \\
    \midrule
    $0.1$   &$59.63$        & $44.63$ \\
    $0.25$  &$61.66$        & $46.57$ \\
    $0.4$   &$\bm{62.20}$   & $47.58$ \\
    $0.5$   &$61.51$        & $47.96$ \\
    $0.75$  &$57.06$        & $\bm{48.04}$ \\
    $0.9$   &$55.99$        & $45.61$ \\
    \bottomrule
  \end{tabular}
  \caption{Our model \emph{Accuracy} as the parameter $\omega$ value changes, in both Flickr30k Entities and ReferIt. The best values are shown in bold. Our model achieves the best-performing results when the \emph{Concept Branch} and the trained modules jointly work to predict the final alignments.
  }
  \label{tab:table_omega}
\end{table}



% \begin{table}
%   \centering
%   \small
%   \begin{tabular}{lcccc}
%     \toprule
%     &\multicolumn{2}{c}{Flickr30k Entities (\%)} & \multicolumn{2}{c}{ReferIt (\%)} \\
%     \cmidrule(rl{4pt}){2-3} \cmidrule(rl{4pt}){4-5}
%     $\omega$ & Acc. & P. Acc. & Acc. & P. Acc. \\
%     \midrule
%     $0.1$   &$59.63$        &$79.64$      & $34.51$ & $\bm{58.34}$ \\
%     $0.25$  &$61.66$        &$\bm{80.82}$ & $34.60$ & $58.27$ \\
%     $0.4$   &$\bm{62.20}$   &$80.68$      & $\bm{34.61}$ &$58.22$       \\
%     $0.5$   &$61.51$        &$79.42$      & $34.53$ & $58.22$ \\
%     $0.75$  &$57.06$        &$76.54$      & $34.32$ & $58.15$ \\
%     $0.9$   &$55.99$        &$74.96$      & $34.07$ & $58.10$ \\
%     \bottomrule
%   \end{tabular}
%   \caption[Ablation study on prior application for both Flickr30k
%     Entities and ReferIt]{ Ablation study on prior application for
%     both Flickr30k Entities and ReferIt.
%   }
%   \label{tab:ablation_prior}
% \end{table}

==> tables/table_clip.tex <==
\begin{table}[t]
  \footnotesize
  \centering
  \begin{tabular}{ccc}
    \toprule
    Model       & Flickr30k (\%) & ReferIt (\%) \\
    \midrule
    CLIP w/o Projection  & $49.65$ & $38.99$ \\
    CLIP   & $56.89$ & $40.99$ \\
    \midrule
    Our model (without CLIP) & $\bm{62.20}$ & $\bm{48.03}$ \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Accuracy results on Flickr30k Entities and ReferIt test sets, leveraging CLIP's multimodal embeddings.} In \emph{CLIP w/o Projection}, the visual and textual branches simply return CLIP encoded representations of proposals and queries, while \emph{CLIP} applies a non-linear transformation to CLIP encoded representations to match the same size of our model's multimodal space.}
  % We tested CLIP embeddings in two settings: (i) in the first (\emph{CLIP}), the visual and textual branches simply return CLIP encoded representations of proposals and queries, while (ii) the second (\emph{CLIP $+$ Projection}) applies a non-linear transformation to CLIP encoded representations such that they match the same size of our model's. The best values are shown in bold.
  \label{tab:clip}
\end{table}

% % wrapped version
% \begin{wraptable}{r}{0.52\linewidth} 
%   \footnotesize
%   \centering
%   \begin{tabular}{c@{\hspace{1\tabcolsep}}c@{\hspace{1\tabcolsep}}c@{\hspace{1\tabcolsep}}}
%     \toprule
%     \multirow{2}{*}[0pt]{Model}    & Flickr30k  & ReferIt \\
%                                     & Entities (\%) & (\%) \\
%     \midrule
%     CLIP           & $49.65$ & $38.99$ \\
%     CLIP $+$ Projection   & $56.89$ & $40.99$ \\
%     \midrule
%     Our model (without CLIP) & $\bm{62.20}$ & $\bm{48.03}$ \\
%     \bottomrule
%   \end{tabular}
%   \caption{\textbf{Accuracy results on Flickr30k Entities and ReferIt leveraging CLIP's multimodal embeddings.} We tested CLIP embeddings in two settings: (i) in the first (\emph{CLIP}), the visual and textual branches simply return CLIP encoded representations of proposals and queries, while (ii) the second (\emph{CLIP $+$ Projection}) applies a non-linear transformation to CLIP encoded representations such that they match the same size of our model's. The best values are shown in bold.}
%   \label{tab:clip}
% \end{wraptable}

%\begin{table}
%  \footnotesize
%  \centering
%  \begin{tabular}{cccc}
%    \toprule
%    Dataset   & CLIP       & Accuracy & P. Accuracy \\
%    \midrule
%    Flickr30k E. & emb        & 49.65 & 74.52    \\
%    % Flickr30k E. & emb        & 49.77    & 74.63    \\  % (w=0.5)
%    % Flickr30k E. & emb        & 15.60    & 57.63    \\  % (w=1)
%    Flickr30k E. & emb + proj & 56.89    & 77.06    \\       
%    % Flickr30k E. & emb + proj & 56.61    & 76.73    \\   % (w=0.5)
%    % Flickr30k E. & emb + proj &  7.96    & 43.79    \\   % (w=1)
%    \midrule
%    ReferIt   & emb        & 38.99    & 57.94    \\
%    % ReferIt   & emb        & 38.98    & 57.92    \\  % (w=0.5)
%    % ReferIt   & emb        & 10.43    & 29.85    \\  % (w=1)
%    ReferIt   & emb + proj & 40.99    & 57.48    \\
%    % referit   & emb + proj & 40.62    & 58.38    \\   % (w=0.1)
%    % referit   & emb + proj & 40.80    & 58.09    \\   % (w=0.25)
%    % referit   & emb + proj & 40.62    & 57.55    \\   % (w=0.5)
%    % referit   & emb + proj &  38.82   & 57.74    \\   % (w=0.75)
%    % referit   & emb + proj &  38.87   & 56.84    \\   % (w=0.9)
%    % referit   & emb + proj &  3.76    & 27.10    \\   % (w=1)
%    \bottomrule
%  \end{tabular}
%  \caption{\textbf{Results on Flickr30k Entities and ReferIt leveraging state-of-the-art multimodal embeddings.} We tested CLIP embeddings in two settings: (i) \emph{emb}, where visual and textual branch simply return CLIP encoded representations of proposal and queries, while (ii) \emph{emb + proj} applies a non-linear transformation to CLIP encoded representation such that they match the same size of our model's.}
%  \label{tab:clip}
%\end{table}

==> tables/table_fraction_omega.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  \parbox{.49\textwidth}{
    \centering
    \begin{tabular}{lcccc}
    \toprule
    $\omega$ &\multicolumn{1}{c}{Flickr30k Entities (\%)} & \multicolumn{1}{c}{ReferIt (\%)} \\
    \midrule
    $0.1$   &$59.63$        & $44.63$ \\
    $0.25$  &$61.66$        & $46.57$ \\
    $0.4$   &$\bm{62.20}$   & $47.58$ \\
    $0.5$   &$61.51$        & $47.96$ \\
    $0.75$  &$57.06$        & $\bm{48.04}$ \\
    $0.9$   &$55.99$        & $45.61$ \\
    \bottomrule
  \end{tabular}
  \caption{
    \textbf{Accuracy results on Flickr30k Entities and ReferIt test sets varying the $\omega$ hyper-parameter.} The best values are shown in bold. Our model achieves the best-performing results when the \emph{Concept Branch} and the trained modules jointly work to predict the final alignments. \label{tab:table_omega}}
  }
  \hfill
  \parbox{.49\textwidth}{
  \centering
  \begin{tabular}{lcc}
    \toprule
    Tr. Fraction &\multicolumn{1}{c}{Flickr30k Entities (\%)} & \multicolumn{1}{c}{ReferIt (\%)} \\
    \midrule
    5\%         &$57.20$        &$41.02$ \\
    10\%        &$60.72$        &$42.67$ \\
    50\%        &$61.49$        &$47.68$ \\
    100\%       &$\bm{62.20}$   &$\bm{48.04}$ \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Accuracy results on Flickr30k Entities and ReferIt test sets training our model with different fractions of the training set.} The best values are shown in bold. Our model presents competitive results even when trained with just 5\% of the training set data.}
  \label{tab:table_fraction_results}
  }
\end{table}
